Joint reconstruction strategy for structured illumination microscopy with unknown illuminations

The blind structured illumination microscopy (SIM) strategy proposed in (Mudry et al., 1992) is fully re-founded in this paper, unveiling the central role of the sparsity of the illumination patterns in the mechanism that drives super-resolution in the method. A numerical analysis shows that the resolving power of the method can be further enhanced with optimized one-photon or two-photon speckle illuminations. A much improved numerical implementation is provided for the reconstruction problem under the image positivity constraint. This algorithm rests on a new preconditioned proximal iteration faster than existing solutions, paving the way to 3D and real-time 2D reconstruction

==> abrege.tex <==
% TEX 7(ascii) bits
%
% ABREGE.tex
% LaTeX document
% Author: J.I. 
% Date  : Juillet 1996
%
% Raccourcis d'expressions tr\`es usit\'ees
%
% Derniere modif le 10-07-96
%

% Raccourci pour \XS
\def\XS{\xspace}

%%%%%%%%%%%%%%%%%%% Pour definir nouvelle commande de changement de taille
\RequirePackage{ifthen}
\RequirePackage{calc}

\newcommand{\taille}[1][\scad]{%
\ifthenelse{#1 = -5}{}{}%
\ifthenelse{#1 = -4}{\tiny}{}%
\ifthenelse{#1 = -3}{\scriptsize}{}%
\ifthenelse{#1 = -2}{\footnotesize}{}%
\ifthenelse{#1 = -1}{\small}{}%
\ifthenelse{#1 = 0}{\normalsize}{}%
\ifthenelse{#1 = 1}{\large}{}%
\ifthenelse{#1 = 2}{\Large}{}%
\ifthenelse{#1 = 3}{\LARGE}{}%
\ifthenelse{#1 = 4}{\huge}{}%
\ifthenelse{#1 = 5}{\Huge}{}}

\newboolean{@serif}
\setboolean{@serif}{true}
\def\scad{-5} % scadefaultsize

\newcounter{taille}
\newcommand{\sca}[2][\scad]{\setcounter{taille}{#1}%
  \ifthenelse{\boolean{@serif}}
  {{\taille[\thetaille]\textsc{#2}}}
  {\setcounter{taille}{\value{taille}-1}{\uppercase{\taille[\thetaille]#2}}}}

% Mise en commentaire rapide !
\def\rem#1{}                    % rem{bla bla bla}

% References automatiquement entre parenthese
\def\reff#1{\XS(\ref{#1})}
\def\refs#1{section~\ref{#1}}
\def\refS#1{Section~\ref{#1}}

\newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}  
% Numéro (pour biblio)
\def\numero{n°}
\def\Numero{N°}

% Majuscules
\def\UP#1{\uppercase{#1}}       % majuscules
\def\up#1{\uppercase{#1}}       % majuscules

% Liste des abreges
\def\adhoc{\textit{ad hoc}\XS}
\def\apost{\textit{a posteriori}\XS}
\def\Apost{\textit{A posteriori}\XS}
\def\APost{\textit{A Posteriori}\XS}
\def\post{\textit{posterior}\XS}
\def\Post{\textit{Posterior}\XS}
\def\afortio{\textit{a fortiori}\XS}
\def\Afortio{\textit{A fortiori}\XS}
\def\aprio{\textit{a priori}\XS}
\def\Aprio{\textit{A priori}\XS}
\def\Cad{C'est-\`a-dire\XS}
\def\cad{c'est-\`a-dire\XS}
\def\coeur{c{\oe}ur\XS}
\def\cf{\textit{cf.}\XS}
\def\cv{\textit{curriculum vit\ae}\XS}
\def\Cv{\textit{Curriculum vit\ae}\XS}
\def\CV{\textit{Curriculum Vit\ae}\XS}
\def\eg{\textit{e.g.,}\XS}
\def\etal{\textit{et al.}\XS}
\def\etc{\textit{etc}\XS}
\def\etcoll{{\textit et coll.}\XS}
\def\idem{\textit{idem}\XS}
\def\ie{\textit{i.e.,}\XS}
\def\IFF{\textit{if and only if}\XS}
\def\iid{i.i.d.\XS}
\def\infine{\textit{in fine}\XS}
\def\insit{\textit{in situ}\XS}
\def\inviv{\textit{in vivo}\XS}
\def\oeuvre{{\oe}uvre\XS}
\def\oeuvres{{\oe}uvres\XS}
\def\recto{\textit{recto}\XS}
\def\Toeplitz{T{\oe}plitz\XS}
\def\vav{vis-\`a-vis\XS}
\def\via{\textit{via}\XS}
\def\vic{\textit{vice-versa}\XS}
\def\verso{\textit{verso}\XS}
%\def\vitae{\textit{vit\ae}\XS}
\def\vs{\textit{vs}\XS}
\def\versus{\textit{versus}\XS}
\def\ssi{\textit{si et seulement si}\XS}
\def\strsen{\textit{stricto sensu}\XS}
\def\wrt{w.r.t.\XS}

\def\ier{$^{\text{\small er}}$\XS}
\def\iere{$^{\text{\small re}}$\XS}
\def\ieme{$^{\text{\small e}}$\XS}

\def\primo{\ensuremath{1^{\oD}}\XS}
\def\secundo{\ensuremath{2^{\oD}}\XS}
\def\tertio{\ensuremath{3^{\oD}}\XS}
\def\quatro{\ensuremath{4^{\oD}}\XS}


\newcommand{\art}[1][\scad]{\sca[#1]{art}\XS}
\newcommand{\cnd}[1][\scad]{\sca[#1]{cnd}\XS}
\newcommand{\ndt}[1][\scad]{\sca[#1]{ndt}\XS}
\newcommand{\gnc}[1][\scad]{\sca[#1]{gnc}\XS}
\newcommand{\mfa}[1][\scad]{\sca[#1]{mfa}\XS}
\newcommand{\map}[1][\scad]{\sca[#1]{map}\XS}

\newcommand{\icm}[1][\scad]{\sca[#1]{icm}\XS}
\newcommand{\icd}[1][\scad]{\sca[#1]{icd}\XS}
\newcommand{\rsb}[1][\scad]{\sca[#1]{rsb}\XS}
\newcommand{\snr}[1][\scad]{\sca[#1]{snr}\XS}

\newcommand{\dess}[1][\scad]{\sca[#1]{dess}\XS}
\newcommand{\dea}[1][\scad]{\sca[#1]{dea}\XS}
\newcommand{\deug}[1][\scad]{\sca[#1]{deug}\XS}
\newcommand{\deust}[1][\scad]{\sca[#1]{deust}\XS}
\newcommand{\iut}[1][\scad]{\sca[#1]{iut}\XS}
\newcommand{\iup}[1][\scad]{\sca[#1]{iup}\XS}

\newcommand{\eea}[1][\scad]{\sca[#1]{eea}\XS}
\def\EEA{\'Electronique \'Electrotechnique Automatique\XS}
\newcommand{\ats}[1][\scad]{\sca[#1]{ats}\XS}
\def\ATS{Automatique et Traitement du Signal\XS}

\newcommand{\te}[1][\scad]{\sca[#1]{te}\XS}
\def\TE{travaux d'études\XS}
\newcommand{\td}[1][\scad]{\sca[#1]{td}\XS}
\def\TD{travaux dirigés\XS}
\newcommand{\tp}[1][\scad]{\sca[#1]{tp}\XS}
\def\TP{travaux pratiques\XS}
%\newcommand{\tdao}[1][\scad]{\sca[#1]{tdao}\XS}
\def\TDAO{travaux dirigés assistés sur ordinateur\XS}
\newcommand{\tdao}[1][\scad]{\sca[#1]{tdao}\XS}
\def\ts{traitement du signal\XS}
\def\TS{Traitement du Signal\XS}

\newcommand{\gbm}[1][\scad]{\sca[#1]{gbm}\XS}
\newcommand{\irmf}[1][\scad]{\sca[#1]{irm-f}\XS}
\newcommand{\irm}[1][\scad]{\sca[#1]{irm}\XS}
\newcommand{\rmn}[1][\scad]{\sca[#1]{rmn}\XS}
\newcommand{\eeg}[1][\scad]{\sca[#1]{eeg}\XS}
\newcommand{\meg}[1][\scad]{\sca[#1]{meg}\XS}

\newcommand{\pc}[1][\scad]{\sca[#1]{pc}\XS}
% Operating Systemes 
\newcommand{\linux}[1][\scad]{\sca[#1]{Linux}\XS}
\newcommand{\unix}[1][\scad]{\sca[#1]{Unix}\XS}
\newcommand{\msdos}[1][\scad]{\sca[#1]{msdos}\XS}
\newcommand{\sunos}[1][\scad]{\sca[#1]{Sunos}\XS}
\newcommand{\hupux}[1][\scad]{\sca[#1]{hp-ux}\XS}
\newcommand{\vms}[1][\scad]{\sca[#1]{vms}\XS}
\newcommand{\solaris}[1][\scad]{\sca[#1]{Solaris}\XS}
\newcommand{\winnt}[1][\scad]{\sca[#1]{Windows-nt}\XS}
\newcommand{\vmware}[1][\scad]{\sca[#1]{vmware}\XS}
\newcommand{\win}[1][\scad]{\sca[#1]{Windows}\XS}

% Calcul scientifique
\newcommand{\labview}[1][\scad]{\sca[#1]{Labview}\XS}
\newcommand{\matlab}[1][\scad]{\sca[#1]{Matlab}\XS}
\newcommand{\maple}[1][\scad]{\sca[#1]{Maple}\XS}
\newcommand{\mathe}[1][\scad]{\sca[#1]{Mathematica}\XS}
\newcommand{\idl}[1][\scad]{\sca[#1]{Idl}\XS}

% langages
\newcommand{\cmex}[1][\scad]{\sca[#1]{Cmex}\XS}
\newcommand{\pascal}[1][\scad]{\sca[#1]{Pascal}\XS}
\newcommand{\java}[1][\scad]{\sca[#1]{Java}\XS}
\newcommand{\lisp}[1][\scad]{\sca[#1]{Lisp}\XS}
\newcommand{\forts}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 77}\XS}
\newcommand{\fortq}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 90}\XS}
\newcommand{\ada}[1][\scad]{\sca[#1]{Ada}\XS}
\newcommand{\eiffel}[1][\scad]{\sca[#1]{Eiffel}\XS}
\newcommand{\tcsh}[1][\scad]{\sca[#1]{tcsh}\XS}
\newcommand{\bash}[1][\scad]{\sca[#1]{bash}\XS}
\newcommand{\lgc}[1][\scad]{\sca[#1]{C}\XS}
\newcommand{\cpp}[1][\scad]{\sca[#1]{C}{\footnotesize ++}\XS}

\def\crec{chargé de recherches\XS}
\def\Crec{Chargé de recherches\XS}
\def\dr{directeur de recherches\XS}
\def\Dr{Directeur de recherches\XS}


% congres
\newcommand{\gretsi}[1][\scad]{\sca[#1]{gretsi}\XS}
\newcommand{\maxent}[1][\scad]{\sca[#1]{maxent}\XS}
\newcommand{\icip}[1][\scad]{\sca[#1]{icip}\XS}
\newcommand{\icassp}[1][\scad]{\sca[#1]{icassp}\XS}
\newcommand{\spie}[1][\scad]{\sca[#1]{spie}\XS}
\newcommand{\gdr}[1][\scad]{\sca[#1]{gdr--prc~isis}\XS}
\newcommand{\rfia}[1][\scad]{\sca[#1]{rfia}\XS}
\newcommand{\eusipco}[1][\scad]{\sca[#1]{eusipco}\XS}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Ajout de famouss.tex
% modif le 25/5/2000 Phiphi
% GPInuts - Famous people - VIP
%
\newcommand{\beaunom}[4][0]{{\taille[#1]#2 \uppercase{#3}}%
{\sca[#1]{#4}}\XS}

%\newcommand{\MA}[1][\scad]{{\taille[#1]Marc \uppercase{A}}% 
%{\sca[#1]{llain}\XS}}
\newcommand{\MA}[1][\scad]{\beaunom[#1]{Marc}{A}{llain}}
\newcommand{\AB}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc}}
\newcommand{\ABF}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc~--~Fusco}}
\newcommand{\AC}[1][\scad]{\beaunom[#1]{Alain}{C}{oulais}}
\newcommand{\AH}[1][\scad]{\beaunom[#1]{Alain}{H}{erment}}
\newcommand{\AMD}[1][\scad]{\beaunom[#1]{Ali}{M}{ohammad--Djafari}}
\newcommand{\AR}[1][\scad]{\beaunom[#1]{Andrea}{R}{idolfi}}
\newcommand{\CH}[1][\scad]{\beaunom[#1]{Christian}{H}{einrich}}
\newcommand{\CS}[1][\scad]{\beaunom[#1]{Charles}{S}{oussen}}
\newcommand{\DLB}[1][\scad]{\beaunom[#1]{Denis}{L}{e Bihan}}
\newcommand{\FC}[1][\scad]{\beaunom[#1]{Fr\'ed\'eric}{C}{hampagnat}}
\newcommand{\FL}[1][\scad]{\beaunom[#1]{Franck}{L}{etimonier}}
\newcommand{\FV}[1][\scad]{\beaunom[#1]{Francisco}{V}{arela}}
\newcommand{\FDU}[1][\scad]{\beaunom[#1]{Fr\'ed\'eric}{D}{ublanchet}}
\newcommand{\GDE}[1][\scad]{\beaunom[#1]{Guy}{D}{emoment}}
\newcommand{\GLB}[1][\scad]{\beaunom[#1]{Guy Le}{B}{esnerais}}
\newcommand{\HC}[1][\scad]{\beaunom[#1]{Herv\'e}{C}{arfantan}}
\newcommand{\JFB}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{B}{ercher}}
\newcommand{\JFG}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{G}{iovannelli}}
\newcommand{\JFM}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{M}{angin}}
\newcommand{\JI}[1][\scad]{\beaunom[#1]{J\'er\^ome}{I}{dier}}
\newcommand{\JBP}[1][\scad]{\beaunom[#1]{Jean-Baptiste}{P}{oline}}
\newcommand{\MF}[1][\scad]{\beaunom[#1]{Marc}{F}{ayolle}}
\newcommand{\Mimi}[1][\scad]{\beaunom[#1]{Myriam}{F}{iani}}
\newcommand{\MN}[1][\scad]{\beaunom[#1]{Mila}{N}{ikolova}}
\newcommand{\PC}[1][\scad]{\beaunom[#1]{Philippe}{C}{iuciu}}
\newcommand{\LG}[1][\scad]{\beaunom[#1]{Line}{G}{arnero}}
\newcommand{\SB}[1][\scad]{\beaunom[#1]{St\'ephane}{B}{rette}}
\newcommand{\SBA}[1][\scad]{\beaunom[#1]{Sylvain}{B}{ailet}}
\newcommand{\RB}[1][\scad]{\beaunom[#1]{Redha}{B}{oubertakh}}
\newcommand{\TM}[1][\scad]{\beaunom[#1]{Thierry}{M}{artin}}
\newcommand{\VS}[1][\scad]{\beaunom[#1]{Vincent}{S}{amson}}
\newcommand{\YG}[1][\scad]{\beaunom[#1]{Yves}{G}{oussard}}
\newcommand{\KS}[1][\scad]{\beaunom[#1]{Ken}{S}{auer}}
\newcommand{\HS}[1][\scad]{\beaunom[#1]{Hichem}{S}{noussi}}

% Acronymes et raccourcis
%
\def\ATER{Attach\'e temporaire d'enseignement et de recherche}
\newcommand{\ater}[1][\scad]{\sca[#1]{ater}\xspace}
\def\ADDOC{Agir pour les Doctorants et les jeunes Docteurs\XS}
\newcommand{\addoc}[1][\scad]{\sca[#1]{addoc}\XS}

\def\CdO{Centre d'Orsay\XS}

\def\CEA{Commissariat à l'\'Enegie Atomique\XS}
\newcommand{\cea}[1][\scad]{\sca[#1]{cea}\XS}
\newcommand{\dam}[1][\scad]{\sca[#1]{dam}\XS}
\def\DRM{D\'epartement de Recherche M\'edicale\XS}
\newcommand{\drm}[1][\scad]{\sca[#1]{drm}\XS}
\def\DSV{Direction des Sciences du Vivant\XS}
\newcommand{\dsv}[1][\scad]{\sca[#1]{dsv}\XS}
\newcommand{\leti}[1][\scad]{\sca[#1]{leti}\XS}
\def\SHFJ{Service Hospitalier Frédéric Joliot\XS}
\newcommand{\shfj}[1][\scad]{\sca[#1]{shfj}\XS}
\def\UNAF{Unit\'e de Neuroimagerie Anatomo Foncxtionnelle\XS}
\newcommand{\unaf}[1][\scad]{\sca[#1]{unaf}\XS}


\newcommand{\chu}[1][\scad]{\sca[#1]{chu}\XS}
\def\CHU{Centre Hospitalier Universitaire\XS}
\def\salpe{Salpétrière\XS}
\def\hsalpe{Hôpital de la Salpétrière\XS}
\def\pisalpe{Pitié-Salpétrière\XS}
\def\gpisalpe{Groupe Pitié-Salpétrière\XS}

\def\CNRS{Centre National de la Recherche Scientifique\XS}
\newcommand{\cnrs}[1][\scad]{\sca[#1]{cnrs}\XS}

\newcommand{\edf}[1][\scad]{\sca[#1]{edf}\XS}
\def\EDF{\'Electricité de France\XS}

\def\ENSTA{\'Ecole Nationale Sup\'erieure de Techniques Avanc\'ees\XS}
\newcommand{\ensta}[1][\scad]{\sca[#1]{ensta}\XS}
\def\ESIEA{\'Ecole Supérieure d'Informatique \'Electronique Automatique\XS}
\newcommand{\esiea}[1][\scad]{\sca[#1]{esiea}\XS}
\newcommand{\ensea}[1][\scad]{\sca[#1]{ensea}\XS}


\def\GPI{Groupe Probl\`emes Inverses\XS}
\newcommand{\gpi}[1][\scad]{\sca[#1]{gpi}\XS}

\def\INSERM{Institut National pour la Sant\'e et la Recherche M\'edicale\XS}
\newcommand{\inserm}[1][\scad]{\sca[#1]{inserm}\XS}

\def\CNAM{Conservatoire National des Arts et Métiers\XS}
\newcommand{\cnam}[1][\scad]{\sca[#1]{cnam}\XS}

\def\INRIA{Institut National de Recherche et Informatique et Automatique\XS}
\newcommand{\inria}[1][\scad]{\sca[#1]{inria}\XS}

\def\IAS{Institut d'Astrophysique Spatiale\XS}
\newcommand{\ias}[1][\scad]{\sca[#1]{ias}\XS}

\newcommand{\ipsn}[1][\scad]{\sca[#1]{ipsn}\XS}
\def\IPSN{Institut de Protection et de Sureté Nucléaire\XS}

\def\LSS{Laboratoire des Signaux et Syst\`emes\XS}
\newcommand{\lss}[1][\scad]{\sca[#1]{l{\footnotesize 2}s}\XS}

\def\LIMSI{Laboratoire d'Informatique pour la Mécanique et les Sciences de l'Ingénieur\XS}
\newcommand{\limsi}[1][\scad]{\sca[#1]{limsi-cnrs}\XS}

\def\ONERA{Office National d'\'Etudes et de Recherches A\'erospatiales\XS}
\newcommand{\onera}[1][\scad]{\sca[#1]{on\'era}\XS}

\def\MDC{Ma\^\i tre de conf\'erences\XS}
\def\MDCs{Ma\^\i tres de conf\'erences\XS}
\newcommand{\mdc}[1][\scad]{\sca[#1]{mdc}\XS}

\newcommand{\UND}[1][\scad]{Université de Notre Dame, \sca[#1]{usa}\XS}

\def\UPS{Universit\'e de Paris-Sud\XS}
\newcommand{\ups}[1][\scad]{\sca[#1]{ups}\XS}
\newcommand{\upxi}[1][\scad]{\sca[#1]{upxi}\XS}

% Unites Thomson
\newcommand{\thomair}[1][\scad]{\sca[#1]{Thomson-csf Airsys}\XS}
\newcommand{\oscar}[1][\scad]{\sca[#1]{Oscar}\XS}
\newcommand{\thomrcm}[1][\scad]{\sca[#1]{Thomson-rcm}\XS}

% Unite propre de recherche
\newcommand{\upr}[1][\scad]{\sca[#1]{upr}\XS}
% LENA, lena upr640,...
\newcommand{\uprlen}[1][\scad]{\sca[#1]{upr}{\footnotesize 640}\XS}
\def\LENA{Laboratoire d'Encéphalographie et de Neurophysiologie Appliquée\XS}
\newcommand{\lena}[1][\scad]{\sca[#1]{lena}\XS}
% Nous
\def\GsY{Gif--sur--Yvette\XS}
\newcommand{\ESE}[1][\scad]{\sca[#1]{sup\'elec}\XS}

\def\adrshort{\ESE, Plateau de Moulon, 91192 Gif--sur--Yvette Cedex\XS}
%\def\adresse{\ESE, Plateau de Moulon, 91192 Gif--sur--Yvette Cedex, France\XS}
\newcommand{\hiercea}[1][\scad]{\dsv[#1]/\drm[#1]/\shfj[#1]\XS}

\newcommand{\adresse}[1][\scad]{\ESE[#1], Plateau de Moulon, 91192 Gif--sur--Yvette Cedex, France\XS}
\newcommand{\adresscea}[1][\scad]{4 Place du Général Leclerc, 91406 Orsay Cedex, France\XS}
\newcommand{\tutelle}[1][\scad]{\cnrs[#1]~--~\ESE[#1]~--~\ups[#1]}
%\newcommand{\tutelle}[1][\scad]{\sca[#1]{Cnrs~--~Sup\'elec~--~Ups}}
\def\ALSS{\LSS~(\tutelle)\\\adresse}
\def\ALSSun{\LSS (\tutelle) \adresse}
%


% ---------------------------------------------------- 
% Modele d'en-tete par A. Mohammad-Djafari et J. Idier 
% ---------------------------------------------------- 
%
\def\helvnormal#1{{\fontfamily{phv}\fontsize{11}{14pt}\selectfont #1}}
\def\helvfoot  #1{{\fontfamily{phv}\fontsize{9}{14pt} \selectfont #1}}
\def\helvscript#1{{\fontfamily{phv}\fontsize{8}{14pt} \selectfont #1}}
%
\newcommand{\entete}[5][Nom.Pr\'enom]{
%%%%%%\def\entete#1#2#3#4#5{%
\helvscript{\renewcommand{\arraystretch}{.8}
\begin{tabular}{c} Supélec
\\--------\end{tabular} \hfill
\begin{tabular}{c}Centre national de la recherche scientifique          \\
--------\end{tabular} \hfill
\begin{tabular}{c}\UPS  \\--------\end{tabular}} \\[-.4cm]%
%
\begin{center}\helvnormal{\textbf{LABORATOIRE DES SIGNAUX \& SYST\`EMES}}\\%
\helvfoot{Unit\'e mixte de recherche n$^{\rm o}$ 8506\\%
Sup\'elec, plateau de Moulon, 
3 rue Joliot-Curie, 91192 \sca[-3]{Gif--sur--Yvette} Cedex (France)\\%
T\'el\'ephone\,: 01 69 85 17 12 --- 
T\'el\'ecopie\,: 01 69 85 17 65 --- 
Courriel\,: {#1}@lss.supelec.fr}%
\\[0.5cm]\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{V/R\'ef.\,: #2} & \helvscript{\sca[-3]{Gif}, le} #5\\%
\helvscript{N/R\'ef.\,: #3} \\%
\helvscript{Objet\,: #4}%
\end{tabular}
} 

\newcommand{\inhead}[5][Name.Surname]{
%%%%%%\def\entete#1#2#3#4#5{%
\helvscript{\renewcommand{\arraystretch}{.8}
\begin{tabular}{c} Supélec
\\--------\end{tabular} \hfill
\begin{tabular}{c}Centre national de la recherche scientifique  \\
--------\end{tabular} \hfill
\begin{tabular}{c}\UPS  \\--------\end{tabular}} \\[-.4cm]%
%
\begin{center}\helvnormal{\textbf{LABORATOIRE DES SIGNAUX \& SYST\`EMES}}\\%
\helvfoot{Unit\'e mixte de recherche n$^{\rm o}$ 8506\\%
Sup\'elec, plateau de Moulon, 
3 rue Joliot-Curie, 91192 \sca[-3]{Gif--sur--Yvette} Cedex (France)\\%
Telephone: 01 69 85 17 12 --- 
Fax: 01 69 85 17 65 --- 
E-mail: {#1}@lss.supelec.fr}%
\\[0.5cm]\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{Y/Ref.: #2} & \helvscript{\sca[-3]{Gif}, } #5\\%
\helvscript{O/Ref.: #3} \\%
\helvscript{Subject: #4}%
\end{tabular}
} 



==> alphabet.tex <==
% Document LaTeX        Auteur : Guy Le Besnerais       Date : 25/05/94
% Modification : J.-F. Gio      (15/09/95)
%                               J.I. (format Latex 2e, taille adaptative 22/03/99)
%                                    (fonte blackboard 27/08/99)

% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% c pour cursif : \Ac
% bb pour blackboard : \Abb
% Capitale pour capitale : \Lambda

\typeout{\space}
\typeout{\space\space\space\space Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{\space\space\space\space (necessite les packages xspace, amsmath, bbm)}
\typeout{\space}

\RequirePackage{amsmath}
\RequirePackage{xspace}
\RequirePackage{bbm}

%-------------------------------------------

% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)           
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)           
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif
\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)

%-------------------------------------------

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  %\def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}


% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}\XS}   \def\Acb{{\scb{A}}\XS}
\def\Bc{{\scu{B}}\XS}   \def\Bcb{{\scb{B}}\XS}
\def\Cc{{\scu{C}}\XS}   \def\Ccb{{\scb{C}}\XS}
\def\Dc{{\scu{D}}\XS}   \def\Dcb{{\scb{D}}\XS}
\def\Ec{{\scu{E}}\XS}   \def\Ecb{{\scb{E}}\XS}
\def\Fc{{\scu{F}}\XS}   \def\Fcb{{\scb{F}}\XS}
\def\Gc{{\scu{G}}\XS}   \def\Gcb{{\scb{G}}\XS}
\def\Hc{{\scu{H}}\XS}   \def\Hcb{{\scb{H}}\XS}
\def\Ic{{\scu{I}}\XS}   \def\Icb{{\scb{I}}\XS}
\def\Jc{{\scu{J}}\XS}   \def\Jcb{{\scb{J}}\XS}
\def\Kc{{\scu{K}}\XS}   \def\Kcb{{\scb{K}}\XS}
\def\Lc{{\scu{L}}\XS}   \def\Lcb{{\scb{L}}\XS}
\def\Mc{{\scu{M}}\XS}   \def\Mcb{{\scb{M}}\XS}
\def\Nc{{\scu{N}}\XS}   \def\Ncb{{\scb{N}}\XS}
\def\Oc{{\scu{O}}\XS}   \def\Ocb{{\scb{O}}\XS}
\def\Pc{{\scu{P}}\XS}   \def\Pcb{{\scb{P}}\XS}
\def\Qc{{\scu{Q}}\XS}   \def\Qcb{{\scb{Q}}\XS}
\def\Rc{{\scu{R}}\XS}   \def\Rcb{{\scb{R}}\XS}
\def\Sc{{\scu{S}}\XS}   \def\Scb{{\scb{S}}\XS}
\def\Tc{{\scu{T}}\XS}   \def\Tcb{{\scb{T}}\XS}
\def\Uc{{\scu{U}}\XS}   \def\Ucb{{\scb{U}}\XS}
\def\Vc{{\scu{V}}\XS}   \def\Vcb{{\scb{V}}\XS}
\def\Wc{{\scu{W}}\XS}   \def\Wcb{{\scb{W}}\XS}
\def\Xc{{\scu{X}}\XS}   \def\Xcb{{\scb{X}}\XS}
\def\Yc{{\scu{Y}}\XS}   \def\Ycb{{\scb{Y}}\XS}
\def\Zc{{\scu{Z}}\XS}   \def\Zcb{{\scb{Z}}\XS}


% ALPHABET DROIT EN MATHS, taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT, taille adaptative

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% Nouveau (08/99) : ALPHABET BLACKBOARD, taille adaptative

\def\Abb{{\sbl{A}}\XS}  \def\abb{{\sbl{a}}\XS}
\def\Bbb{{\sbl{B}}\XS}  \def\bbb{{\sbl{b}}\XS}
\def\Cbb{{\sbl{C}}\XS}  \def\cbb{{\sbl{c}}\XS}
\def\Dbb{{\sbl{D}}\XS}  \def\dbb{{\sbl{d}}\XS}
\def\Ebb{{\sbl{E}}\XS}  \def\ebb{{\sbl{e}}\XS}
\def\Fbb{{\sbl{F}}\XS}  \def\fbb{{\sbl{f}}\XS}
\def\Gbb{{\sbl{G}}\XS}  \def\gbb{{\sbl{g}}\XS}
\def\Hbb{{\sbl{H}}\XS}  \def\hbb{{\sbl{h}}\XS}
\def\Ibb{{\sbl{I}}\XS}  \def\ibb{{\sbl{i}}\XS}
\def\Jbb{{\sbl{J}}\XS}  \def\jbb{{\sbl{j}}\XS}
\def\Kbb{{\sbl{K}}\XS}  \def\kbb{{\sbl{k}}\XS}
\def\Lbb{{\sbl{L}}\XS}  \def\lbb{{\sbl{l}}\XS}
\def\Mbb{{\sbl{M}}\XS}  \def\mbb{{\sbl{m}}\XS}
\def\Nbb{{\sbl{N}}\XS}  \def\nbb{{\sbl{n}}\XS}
\def\Obb{{\sbl{O}}\XS}  \def\obb{{\sbl{o}}\XS}
\def\Pbb{{\sbl{P}}\XS}  \def\pbb{{\sbl{p}}\XS}
\def\Qbb{{\sbl{Q}}\XS}  \def\qbb{{\sbl{q}}\XS}
\def\Rbb{{\sbl{R}}\XS}  \def\rbb{{\sbl{r}}\XS}
\def\Sbb{{\sbl{S}}\XS}  \def\sbb{{\sbl{s}}\XS}
\def\Tbb{{\sbl{T}}\XS}  \def\tbb{{\sbl{t}}\XS}
\def\Ubb{{\sbl{U}}\XS}  \def\ubb{{\sbl{u}}\XS}
\def\Vbb{{\sbl{V}}\XS}  \def\vbb{{\sbl{v}}\XS}
\def\Wbb{{\sbl{W}}\XS}  \def\wbb{{\sbl{w}}\XS}
\def\Xbb{{\sbl{X}}\XS}  \def\xbb{{\sbl{x}}\XS}
\def\Ybb{{\sbl{Y}}\XS}  \def\ybb{{\sbl{y}}\XS}
\def\Zbb{{\sbl{Z}}\XS}  \def\zbb{{\sbl{z}}\XS}


% ALPHABET GREC GRAS italique, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}      \def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\varkappab   {{\sbmm{\varkappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}     \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}         \def\Xib       {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}         \def\Pib       {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}   \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib      {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib      {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}   \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}


% CHIFFRES
% Gras et Blackboard, taille adaptative

\def\zerob   {{\sbv{0}}\XS}        \def\zerobb   {{\sbl{O}}\XS}
\def\unb     {{\sbv{1}}\XS}        \def\unbb     {{\sbl{1}}\XS}
\def\deuxb   {{\sbv{2}}\XS}        \def\deuxbb   {{\sbl{2}}\XS}
\def\troisb  {{\sbv{3}}\XS}        \def\troisbb  {{\sbl{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}        \def\quatrebb {{\sbl{4}}\XS}
\def\cinqb   {{\sbv{5}}\XS}        \def\cinqbb   {{\sbl{5}}\XS}
\def\sixb    {{\sbv{6}}\XS}        \def\sixbb    {{\sbl{6}}\XS}
\def\septb   {{\sbv{7}}\XS}        \def\septbb   {{\sbl{7}}\XS}
\def\huitb   {{\sbv{8}}\XS}        \def\huitbb   {{\sbl{8}}\XS}
\def\neufb   {{\sbv{9}}\XS}        \def\neufbb   {{\sbl{9}}\XS}


% QUELQUES ENSEMBLES

\def\eC{\Cbb}
\def\eE{\Ebb}
\def\eN{\Nbb}
\def\eQ{\Qbb}
\def\eR{\Rbb}
\def\eZ{\Zbb}



==> beginend.tex <==
% TEX 7(ascii) bits
% BEGINEND.tex                          LaTeX document
% Author: J.I.          Date : 07/96    Derniere modif le 10/07/96
% Raccourcis des \begin et \end, d'apr\`es les Grands Anciens
% Modification provisoire le 12/02/97 sur \beq#1\eeq --->
% ---> Compatibilit\'e avec Amsmath.sty

\def\babs{\begin{abstract}}             \def\eabs{\end{abstract}}
\def\barr{\begin{array}}                \def\earr{\end{array}}
\def\bcc{\begin{center}}                \def\ecc{\end{center}}
\def\cl#1{\centerline{#1}}
\def\bdes{\begin{description}}          \def\edes{\end{description}}
\def\bdoc{\begin{document}}             \def\edoc{\end{document}}
\def\ben{\begin{enumerate}}             \def\een{\end{enumerate}}
\def\beqn{\begin{eqnarray}}             \def\eeqn{\end{eqnarray}}
\def\beqnl#1{\beqn\label{#1}}           \def\eeqnl#1{\label{#1}\eeqn}
\def\beqnx{\begin{eqnarray*}}           \def\eeqnx{\end{eqnarray*}}
\def\bseqn{\begin{subeqnarray}}         \def\eseqn{\end{subeqnarray}}
%
\def\beq#1\eeq{\begin{equation}#1\end{equation}}
%\def\beq{\begin{equation}}             \def\eeq{\end{equation}}
%\def\beql#1{\beq\label{#1}}            \def\eeql#1{\label{#1}\eeq}
%
\def\bal#1\eal{\begin{align}#1\end{align}}
\def\balx#1\ealx{\begin{align*}#1\end{align*}}
%
\def\beqx{$$}                           \def\eeqx{$$}
\def\bfig{\protect\begin{figure}}       \def\efig{\protect\end{figure}}
\def\bfigx{\protect\begin{figure*}}     \def\efigx{\protect\end{figure*}}
\def\bfigt{\protect\begin{figurette}}   \def\efigt{\protect\end{figurette}}
\def\bfl{\begin{flushleft}}             \def\efl{\end{flushleft}}
\def\bfr{\begin{flushright}}            \def\efr{\end{flushright}}
\def\bit{\begin{itemize}}               \def\eit{\end{itemize}}
\def\bmi{\begin{minipage}}              \def\emi{\end{minipage}}
\def\bfmi{\begin{fminipage}}            \def\efmi{\end{fminipage}}
\def\bpic{\begin{picture}}              \def\epic{\end{picture}}
\def\bqu{\begin{quote}}                 \def\equ{\end{quote}}
\def\bqun{\begin{quotation}}            \def\equn{\end{quotation}}
\def\bsl{\begin{slide}}                 \def\esl{\end{slide}}
\def\btabb{\begin{tabbing}}             \def\etabb{\end{tabbing}}
\def\btabl{\begin{table}}               \def\etabl{\end{table}}
\def\btablx{\begin{table*}}             \def\etablx{\end{table*}}
\def\btab{\begin{tabular}} %\def\etab{\end{tabular}} Conflit avec eta gras... Elle est pas grasse, ma soeur !
\def\btabu{\begin{tabular}}             \def\etabu{\end{tabular}}
\def\btabx{\begin{tabular*}}            \def\etabx{\end{tabular*}}
\def\bbib{\begin{thebibliography}{999}} \def\ebib{\end{thebibliography}}
\def\bver{\begin{verbatim}}             \def\ever{\end{verbatim}}
\def\bca{\begin{cases}}                  \def\eca{\end{cases}}

